Stochastic Weighted Matching: $(1-\epsilon)$ Approximation

Let $G=(V, E)$ be a given edge-weighted graph and let its {\em realization} $\mathcal{G}$ be a random subgraph of $G$ that includes each edge $e \in E$ independently with probability $p$. In the {\em stochastic matching} problem, the goal is to pick a sparse subgraph $Q$ of $G$ without knowing the realization $\mathcal{G}$, such that the maximum weight matching among the realized edges of $Q$ (i.e. graph $Q \cap \mathcal{G}$) in expectation approximates the maximum weight matching of the whole realization $\mathcal{G}$. In this paper, we prove that for any desirably small $\epsilon \in (0, 1)$, every graph $G$ has a subgraph $Q$ that guarantees a $(1-\epsilon)$-approximation and has maximum degree only $O_{\epsilon, p}(1)$. That is, the maximum degree of $Q$ depends only on $\epsilon$ and $p$ (both of which are known to be necessary) and not for example on the number of nodes in $G$, the edge-weights, etc. The stochastic matching problem has been studied extensively on both weighted and unweighted graphs. Previously, only existence of (close to) half-approximate subgraphs was known for weighted graphs [Yamaguchi and Maehara, SODA'18; Behnezhad et al., SODA'19]. Our result substantially improves over these works, matches the state-of-the-art for unweighted graphs [Behnezhad et al., STOC'20], and essentially settles the approximation factor.

==> expfracmatching.tex <==
\subsection{Construction of an Expected Fractional Matching $x$ on $\mc{Q}$}\label{sec:constructfractional}

In this section, we describe an algorithm that constructs an ``expected fractional matching'' $x$ on $\mc{Q}$ as defined below.

\begin{definition}\label{def:expfractional}
	Let $\mathcal{A}$ be a random process that assigns a fractional value $x_e \in [0, 1]$ to each edge $e$ of a graph $G(V, E)$. We say $x$ is an expected fractional matching if:
	\begin{enumerate}[itemsep=0pt,topsep=5pt]
		\item For each vertex $v$, defining $x_v := \sum_{e \ni v} x_e$ we have $\E[x_v] \leq 1$.
		\item For all subsets $U \subseteq V$ with $|U|\leq 1/\epsilon$, $x(U) \leq \lfloor \frac{|U|}{2} \rfloor$ with probability 1.
	\end{enumerate}
\end{definition}

We emphasize that the definition only requires $\E[x_v] \leq 1$, thus depending on the coin tosses of the process, it may occur that $x_v > 1$, violating the constraints of a normal fractional matching. We will later argue that in our construction, the values of $x_v$'s are sufficiently concentrated around their mean and thus we can turn our expected fractional matching to an actual fractional matching of (almost) the same size.

As described before, we construct an expected fractional matching $x$ on the edges of graph $\mc{Q}$. Note that here the graph $\mc{Q}$ itself is also stochastic. In the construction, we treat crucial and non-crucial edges completely differently.

\smparagraph{Crucial edges.} On the crucial edges, we first construct an integral matching $Z$ using the algorithm of Lemma~\ref{lem:independentmatching}. Once we have $Z$, we define $x$ on crucial edges as follows.

\begin{highlighttechnical}
\vspace{-0.4cm}
\begin{flalign}\label{eq:crucialxe}
	\text{For every crucial edge $e$, } \qquad\qquad x_e := \begin{cases}
    1,& \text{if $e \in Z$ and $e \in Q$,}\\
    0,              & \text{otherwise}.
    \end{cases}
\end{flalign}
\end{highlighttechnical}

Note from Observation~\ref{obs:samplealmostallcrucial} that each crucial edges belong to $Q$ with probability at least $1-\epsilon$. Therefore the construction above (roughly speaking) sets $x_e = 1$ for most of the edges $e$ in $Z$.

\smparagraph{Non-crucial edges.} For defining $x$ on the non-crucial edges, we start with a number of useful definitions. For any edge $e$, define $t_e$ to be the number of matchings $M(\mc{G}_1), \ldots, M(\mc{G}_R)$ that include $e$. Then based on that, define 
\begin{equation}\label{eq:deff}
	f_e := \begin{cases}
		\frac{t_e}{R}, & \text{if $\frac{t_e}{R} \leq \frac{1}{\sqrt{\epsilon R}}$ and $e$ is non-crucial,}\\
		0, & \text{otherwise.}
	\end{cases}
\end{equation}
Note that $f_e$ is a random variable of only the randomization of Algorithm~\ref{alg:sampling}, i.e. it is independent of the realization. Also note that $f_e$ is desirably non-zero only on the edges that belong to graph $Q$. Having defined $f_e$, we define $x_e$ on the non-crucial edges as follows.
\begin{highlighttechnical}
For every non-crucial edge $e$, define
\begin{flalign}\label{eq:noncrucialxe}
	x_e = \begin{cases}
    \frac{f_e}{p_e(1-\Pr[X_v])(1-\Pr[X_u])}, & \text{if $e$ is realized, $u, v \not\in V(Z)$, and $d_C(u, v) \geq \lambda$,}\\
    0,              & \text{otherwise}.
    \end{cases}
\end{flalign}
\end{highlighttechnical}

We note that $\lambda$ in the definition above is the number defined in Lemma~\ref{lem:independentmatching}.

Before concluding this section, let $f_v := \sum_{e \in N : v \in e} f_e$ for each vertex $v$. We note the following properties of $f$, which can be derived directly from the definition above. The proof is given in Section~\ref{sec:proofs}.

\begin{claim}\label{cl:frange}
	It holds that:
	\begin{enumerate}
		\item For every non-crucial edge $e$, $\E[f_e] \leq q_e$.
		\item For every non-crucial edge $e$, $\E[f_e] \geq (1-\epsilon)q_e$.
		\item For every vertex $v$, it always holds that $\sum_{e \ni v} f_e \leq 1$.
		\item For every vertex $v$, $\Pr[f_v > n_v + 0.1\epsilon] \leq (\epsilon p)^{10}$.
	\end{enumerate}
\end{claim}

Consider a non-crucial edge $\{u, v\}$ between two nodes $u$ and $v$ with $d_C(u, v) \geq \lambda$. The probability that $x_e$ is non-zero is $p_e(1-\Pr[X_v])(1-\Pr[X_u])$: Both $u$ and $v$ should be unmatched in $Z$ and $e$ should be realized, and further all these events are independent. This intuitively explains why we set $x_e = \frac{f_e}{p_e(1-\Pr[X_v])(1-\Pr[X_u])}$ if all these conditions hold: We want the denominator to cancel out with this probability so that we get $\E[x_e] = f_e$. We will formalize this intuition in Section~\ref{sec:analysisfractional} where we prove the expected size of $x$ is large.

\subsection{Validity of $x$}\label{sec:validityofx}

In this section, we prove that $x$ is indeed an expected fractional matching of $\mc{Q}$.

First, we prove that $x$ is non-zero only on the edges of $\mc{Q}$. This simply follows from the construction of $x$.

\begin{claim}
	Any edge $e$ with $x_e > 0$ belongs to $\mc{Q}$. That is, $x$ is only non-zero on the set of edges queried by Algorithm~\ref{alg:sampling} that are also realized.
\end{claim}
\begin{proof}
	For any crucial edge $e$, we either have $x_e = 1$ or $x_e = 0$. By definition, if $x_e = 1$ then $e \in Z \cap Q$. By Lemma~\ref{lem:independentmatching}, $Z$ is a matching of {\em realized} crucial edges, i.e. $e \in Z$ implies $e \in \mc{E}$. Therefore, $e \in Z \cap Q$ implies $e \in \mc{E} \cap Q = \mc{Q}$ as desired.
	
	For any non-crucial edge $e$, if $e \not\in Q$, then $f_e = 0$ by definition of $f_e$. Therefore, if $x_e > 0$, then $f_e > 0$ which implies $e \in Q$. Moreover, by (\ref{eq:noncrucialxe}), $x_e > 0$ implies $e$ is realized. Combining these two, we get that if $x_e>0$ then $e \in \mc{Q}$.
\end{proof}

Next, we prove condition (1) of Definition~\ref{def:expfractional}.

\begin{claim}\label{cl:expxvlt1}
	For every vertex $v$, $\E[x_v] \leq 1$.
\end{claim}
\begin{proof}
	Suppose at first that there is an edge $e$ incident to $v$ that belongs to matching $Z$. Then we either have $x_e = 1$ or $x_e = 0$ (depending on whether $e \in Q$ or not). For all other edges $e'$ connected to $v$ (crucial or non-crucial) we have $x_{e'} = 0$ by (\ref{eq:crucialxe}) and (\ref{eq:noncrucialxe}). Therefore if such edge $e$ exists, we indeed have $x_v \leq 1$. For the rest of the proof, we condition on the event that no such edge $e$ exists, i.e. $v \not\in V(Z)$ and prove the claim.
	
	Let $u_1, u_2, \ldots, u_r$ be neighbors of $v$ in graph $G$ such that for all $i \in [r]$: (1) edge $\{v, u_i\}$ is non-crucial, (2) $d_C(v, u_i) \geq \lambda$. Let $e_i := \{v, u_i\}$; we  claim that conditioned on $v \not\in V(Z)$, we have
	\begin{equation}\label{eq:21410238471098412}
	x_v = x_{e_1} + x_{e_2} + \ldots + x_{e_r}.
	\end{equation}
	To see this, fix an edge $e = \{v, u\}$ for some $u \not\in \{u_1, \ldots, u_r\}$. We show that $x_e = 0$, which suffices to prove (\ref{eq:21410238471098412}). First if $e$ is crucial, then $e \not\in Z$ given that $v \not\in V(Z)$; thus according to (\ref{eq:crucialxe}) we set $x_e = 0$. Moreover, if $e$ is non-crucial, the assumption $u \not\in \{u_1, \ldots, u_r\}$ implies $d_C(v, u) < \lambda$ by definition of the set. In this case also, we set $x_e = 0$ according to (\ref{eq:noncrucialxe}); concluding the proof of (\ref{eq:21410238471098412}).
	
	By linearity of expectation applied to (\ref{eq:21410238471098412}), we get
	\begin{equation}\label{eq:612903247}
	\E[x_v \mid v \not\in V(Z)] = \sum_{i=1}^r \E[x_{e_i} \mid v \not\in V(Z)].
	\end{equation}
	Moreover, for any arbitrary $i \in [r]$ we have
	\begin{align}
		\nonumber\E[x_{e_i} \mid v\not\in V(Z)] &= \Pr[u_i \not\in V(Z), e_i \text{ realized} \mid v \not\in V(Z)] \times \frac{\E[f_{e_i}]}{p_{e_i}(1-\Pr[X_v])(1-\Pr[X_{u_i}])}\\
		&= p_{e_i}(1-\Pr[X_{u_i}]) \times \frac{\E[f_{e_i}]}{p_{e_i}(1-\Pr[X_v])(1-\Pr[X_{u_i}])} = \frac{\E[f_{e_i}]}{1-\Pr[X_v]}.\label{eq:7128312098}
	\end{align}
	The second equality above follows from the fact that the event of $e_i$ being realized is independent of $u_i$ or $v$ being in $V(Z)$, as indicated by Lemma~\ref{lem:independentmatching} part 3; and also the fact that $u_i \not\in V(Z)$ and $v \not\in V(Z)$ are also independent from each other due to Lemma~\ref{lem:independentmatching} part 4 combined with the assumption that $d_C(u_i, v) \geq \lambda$. We also note that we have used $\E[f_{e_i}]$ instead of $\E[f_{e_i} \mid v\not\in V(Z)]$ in the equation above since $f_{e_i}$ is only a random variable of the randomization used in Algorithm~\ref{alg:sampling} whereas the matching $Z$ is constructed in Lemma~\ref{lem:independentmatching} independent of the outcome of Algorithm~\ref{alg:sampling}.
	
	Combining (\ref{eq:612903247}) and (\ref{eq:7128312098}) we get
	\begin{equation}\label{eq:421610986201363}
		\E[x_v \mid v\not\in V(Z)] = \sum_{i = 1}^r \frac{\E[f_{e_i}]}{1-\Pr[X_v]} = \frac{1}{1-\Pr[X_v]}\sum_{i=1}^r\E[f_{e_i}].
	\end{equation}	
	From Claim~\ref{cl:frange} part 1, we know $\E[f_{e_i}] \leq q_{e_i}$. Replacing this into the equality above, we get
	$$
		\E[x_v \mid v\not\in V(Z)] \leq \frac{1}{1-\Pr[X_v]} \sum_{i=1}^r q_{e_i} \leq \frac{n_v}{1-\Pr[X_v]}.
	$$
	
	Lemma~\ref{lem:independentmatching} part (2) guarantees that $\Pr[X_v] < c_v$ which implies $1-\Pr[X_v] > 1-c_v$. On the other hand, $c_v + n_v$ is upper bounded by the probability that $v$ is matched in $\opt$, thus $c_v + n_v \leq 1$, implying $n_v \leq 1-c_v$. These, combined with the equation above, gives
	$$
		\E[x_v \mid v\not\in V(Z)] \leq \frac{n_v}{1-\Pr[X_v]} \leq \frac{1-c_v}{1-c_v} = 1.
	$$
	Recalling also that $\E[x_v \mid v\in V(Z)] \leq 1$ as described at the start of the proof, this concludes the proof of the claim that $\E[x_v] \leq 1$.
\end{proof}

Next, we show that condition (2) of Definition~\ref{def:expfractional} also holds for our construction.

\begin{claim}\label{cl:xblossom}
	For all subsets $U \subseteq V$ with $|U|\leq 1/\epsilon$, $x(U) \leq \lfloor \frac{|U|}{2} \rfloor$ with probability 1.
\end{claim}
\begin{proof}
	By definition of $x$, the value of $x_e$ on crucial edges is either 1 or 0. Moreover, the definition also implies that if a vertex $v$ is incident to a crucial edge $e$ with $x_e = 1$, for all other edges $e'$ incident to $v$ we have $x_{e'} = 0$. Call all such vertices {\em integrally matched}. Fix a subset $U$ and let $U'$ be the subset of $U$ excluding its integrally matched vertices. One can easily confirm that if $x(U) > \lfloor |U|/2 \rfloor$, then also $x(U') > \lfloor |U'|/2 \rfloor$. Therefore, either the claim holds, or there should exist a subset with no integrally matched vertices that violates it. Let $U$ be the smallest such subset and observe that $|U| \leq 1/\epsilon$ (otherwise $U$ does not contradict the claim's statement).	
	
	Since $U$ has no integrally matched vertex, for every crucial edge $e$ inside $U$ we have $x_e = 0$ and for every non-crucial edge $e$ inside $U$ by definition (\ref{eq:noncrucialxe}) we have
	$
		x_e \leq \frac{f_e}{p_e (1-\Pr[X_u]) (1-\Pr[X_v])}.
	$
	By definition of $f_e$, it holds that $f_e \leq 1/\sqrt{\epsilon R}$ and by Lemma~\ref{lem:independentmatching} part 2, $\Pr[X_u], \Pr[X_v] \leq 1-\epsilon^2$. Replacing these into the bound above, we get
	$
		x_e \leq \frac{1}{p \times \epsilon^2 \times \epsilon^2 \sqrt{\epsilon R}}.
	$ Noting from Corollary~\ref{cor:thresholds} part 4 that $\tau_- < (\epsilon p)^{50}$ and that $R = 2/\tau_-$, we get $R > 2/(\epsilon p)^{50}$. Replacing this into the previous upper bound on $x_e$, we get that $x_e$ is much smaller than say $\epsilon^3$.
	
	Now since $|U| \leq 1/\epsilon$ there are at most $\binom{|U|}{2} < 1/\epsilon^2$ edges $e$ inside $U$ that can have non-zero $x_e$. For each of these, as discussed above $x_e < \epsilon^3$. Thus we have $x(U) < \epsilon^3 \times 1/\epsilon^2 < 1$ which cannot be larger than $\lfloor |U|/2 \rfloor$ if $|U| \geq 2$ (if $|U| \leq 1$, then there are no edges with both endpoints in $U$ and thus clearly $x(U) = 0$). This contradicts the assumption that $x(U) > \lfloor |U|/2 \rfloor$, implying that there is no such subset. 
\end{proof}

\subsection{The Expected Size of $x$}\label{sec:analysisfractional}

In this section we prove the following.

\begin{lemma}\label{lem:sizeofx}
	It holds that $\E\left[|x| \right] \geq (1-34\epsilon)\opt$.
\end{lemma}

We start by analyzing the size of $x$ on the crucial edges. This is a simple consequence of Lemma~\ref{lem:independentmatching} part 1 which guarantees $\E[Z]\geq q(C)-30\epsilon \opt$ and Observation~\ref{obs:crucialdegree} which guarantees each crucial edge belongs to $Q$ with probability at least $1-\epsilon$.

\begin{claim}\label{cl:sizeofxcrucial}
	It holds that $\E\left[\sum_{e \in C} x_e \right] \geq q(C)-31\epsilon \opt$.
\end{claim}
\begin{proof}
	Denoting $x(C) = \sum_{e \in C} x_e$, we have
	\begin{equation*}
		\E[x(C)] = \E \Big[ \sum_{e \in C} x_e \Big] = \sum_{e \in C} \E[x_e] = \sum_{e \in C} \Pr[e \in Q \text{ and } e \in Z].
	\end{equation*}
	Observe that $Z$ and $Q$ are picked independently as Lemma~\ref{lem:independentmatching} is essentially unaware of $Q$. Therefore, for any crucial edge $e$ we get 
	$$
	\Pr[e \in Q \text{ and } e \in Z] = \Pr[e \in Q] \times \Pr[e \in Z] \geq (1-\epsilon)\Pr[e \in Z],
	$$
	where the latter inequality comes from Observation~\ref{obs:samplealmostallcrucial}. Replacing this to the equality above gives
	$$
	\E[x(C)] \geq (1-\epsilon)\sum_{e \in C} \Pr[e \in Z] = (1-\epsilon)\E[|Z|] \stackrel{\text{Lemma~\ref{lem:independentmatching} part 1}}{\geq} (1-\epsilon) (q(C)-30\epsilon \opt) \geq q(C) - 31\epsilon \opt,
	$$
	completing the proof of the claim.
\end{proof}

To analyze the size of $x$ on the non-crucial edges, we first define $N'$ to be the subset of non-crucial edges $\{u, v\}$ such that $d_C(u, v) \geq \lambda$ and define $q(N') := \sum_{e \in N'} q_e$ and $x(N') := \sum_{e \in N'} x(N')$. Definition of $N'$ is useful since recall from (\ref{eq:noncrucialxe}) that for any $\{u, v\} \in N$ with $d_C(u, v) < \lambda$ (i.e. $\{u, v\} \not\in N'$) we set $x_e = 0$. Therefore only the edges in $N$ that also belong to $N'$ have non-zero $x_e$, implying $x(N) = x(N')$.

\begin{claim}\label{cl:nplarge}
	It holds that $q(N') \geq q(N)-\epsilon q(C)$.
\end{claim}
\begin{proof}
	For any edge $e = \{u, v\}$ in $N \setminus N'$, we choose an arbitrary shortest path $P$ between $u$ and $v$ in graph $C$ and charge the edges of this path. Note that by definition of $N'$, such path between $u$ and $v$ exists and has size less than $\lambda$. Now, take a crucial edge $f$. We denote by $\Phi(f)$ the set of edges in $N \setminus N'$ for which we charge a path consisting $f$. Below, we argue that
	\begin{equation}\label{eq:612398273497}
		|\Phi(f)| \leq 4(1/\tau_+)^{2\lambda} \qquad \forall f \in C.
	\end{equation}
	
	Fix a crucial edge $f$ and an edge $\{u, v\} \in \Phi(f)$. As discussed above, there should be a path of length less than $\lambda$ between $u$ and $v$ in graph $C$ that passes through $f$. This means that $d_C(u, f) < \lambda$ and $d_C(v, f) < \lambda$. Therefore, both $u$ and $v$ are at distance at most $\lambda$ from $f$ in graph $C$. 
	
	Observe that there are at most $2(\Delta_C)^{\lambda}$ vertices in the $\lambda$-neighborhood of $f$ in graph $C$. Thus, there are at most $2(\Delta_C)^{\lambda} \times 2(\Delta_C)^{\lambda} = 4(\Delta_C)^{2\lambda}$ pairs of vertices that can potentially charge $f$, proving $|\Phi(f)| \leq 4(\Delta_C)^{2\lambda} \leq 4(1/\tau_+)^{2\lambda}$ where the latter inequality comes from Observation~\ref{obs:crucialdegree} that $\Delta_C \leq 1/\tau_+$. This concludes the proof of (\ref{eq:612398273497}).
	
	As discussed above, each edge $e \in N \setminus N'$ charges a path in $C$, thus belongs to $\Phi(f)$ of at least one crucial edge $f$. Therefore, we get
	\begin{equation}\label{eq:10234817293478}
		|N \setminus N'| \leq \sum_{f \in C} \Phi(f).
	\end{equation}
	Every edge $e$ in $N \setminus N'$ is non-crucial, i.e. $q_e \leq \tau_-$. Thus:
	\begin{equation}\label{eq:7873241712304912348}
	\sum_{e \in N \setminus N'} q_e \leq \tau_-|N \setminus N'| \stackrel{(\ref{eq:10234817293478})}{\leq} \tau_- \sum_{f \in C} \Phi(f) \stackrel{(\ref{eq:612398273497})}{\leq} 4\tau_- |C|(1/\tau_+)^{2\lambda} \leq 4\tau_- q(C)(1/\tau_+)^{2\lambda+1},
	\end{equation}
	where the last inequality comes from the fact that $q(C) \geq |C| \tau_+$ as for every edge $e \in C$, $q_e \geq \tau_+$.
	
	From Corollary~\ref{cor:thresholds} we have $\tau_- = (\tau_+)^{10g}$ and we have $g \geq \lambda > 1$ by Observation~\ref{obs:ggtlambda}. Thus:
	$$
	 4\tau_- (1/\tau_+)^{2\lambda+1} = 4 (\tau_+)^{10g} (1/\tau_+)^{2\lambda+1} = 4 (\tau_+)^{10g - (2\lambda - 1)} < 4 \tau_+ < \epsilon.
	$$
	Replacing it into inequality (\ref{eq:7873241712304912348}), we get
	$$
	\sum_{e \in N \setminus N'} q_e \leq \epsilon q(C).
	$$
	This concludes the proof since
	$$
		q(N') = \sum_{e \in N'} q_e = \sum_{e \in N \setminus (N \setminus N')} q_e \geq \sum_{e \in N}q_e - \sum_{e \in N \setminus N'} q_e \geq q(N) - \epsilon q(C)
	$$
	as it is desired.
%	Replacing this inequality into 
%	$q(N') = \sum_{e \in N \}= q(N) - \sum_{e \in N' \setminus N} q_e$
%	, we indeed get $q(N') \geq q(N) -\epsilon q(C)$ which concludes the proof.
\end{proof}


\begin{claim}\label{cl:xnpgtqnp}
	It holds that $\E[x(N')] \geq (1-\epsilon) q(N')$.
\end{claim}
\begin{proof}
	By linearity of expectation, we have 
	\begin{equation}\label{eq:16234421340}
	\E[x(N')] = \E \Big[ \sum_{e \in N'} x_e \Big] = \sum_{e \in N'} \E[x_e].
	\end{equation}
	We emphasize that the expectation here is taken over the randomization in Algorithm~\ref{alg:sampling}, the randomization in matching $Z$, and the randomization in realization of non-crucial edges. Specifically, we write $\E_{\alg, Z, \mc{N}}[x_e]$ to emphasize on this.
	
	The randomization of Algorithm~\ref{alg:sampling} determines the value of $f_e$ which is used in defining $x_e$. Let us first condition on $f_e$ and compute $\E_{Z, \mc{N}}[x_e \mid f_e]$. We have
	\begin{equation}\label{eq:89123}
		\E_{Z, \mc{N}}[x_e \mid f_e] = \Pr[e \in \mc{E} \text{ and } u, v \not\in V(Z) \mid f_e] \times  \frac{f_e}{p_e(1-\Pr[X_u])(1-\Pr[X_v])}.
	\end{equation}
	We claim that 
	\begin{equation}\label{eq:5123674182374}
		\Pr[e \in \mc{E} \text{ and } u, v \not\in V(Z) \mid f_e] = p_e(1-\Pr[X_u])(1-\Pr[X_v]).
	\end{equation}
	To see this, first observe that the value of $f_e$ is determined solely by the random realizations taken by Algorithm~\ref{alg:sampling}. In particular, the events $e \in \mc{E}$, and $u, v \not\in V(Z)$ are completely independent of the outcome of Algorithm~\ref{alg:sampling}. This allows us to remove the condition on $f_e$ from the left hand side of (\ref{eq:5123674182374}). Moreover, by Lemma~\ref{lem:independentmatching} part 3, the matching $Z$ is chosen independently from the realization of non-crucial edges, thus events $e \in \mc{E}$ and $u, v \not\in V(Z)$ are independent. 	Finally, the assumption that $e \in N'$, by definition of $N'$, implies that $d_C(u, v) \geq \lambda$. Therefore, by Lemma~\ref{lem:independentmatching} part 4, events $v \in V(Z)$ and $u \in V(Z)$ (and for that matter their complements) are independent. Thus, indeed:
	\begin{align*}
	\Pr[e \in \mc{E} \text{ and } u, v \not\in V(Z) \mid f_e] &= \Pr[e \in \mc{E}] \times \Pr[v \not\in V(Z)] \times \Pr[u \not\in V(Z)]\\
	&= p_e(1-\Pr[X_u])(1-\Pr[X_v]).
	\end{align*}
	Replacing (\ref{eq:5123674182374}) into (\ref{eq:89123}) we get
	\begin{equation*}
		\E_{Z, \mc{N}}[x_e \mid f_e] = p_e(1-\Pr[X_u])(1-\Pr[X_v]) \times \frac{f_e}{p_e(1-\Pr[X_u])(1-\Pr[X_v])} = f_e.
	\end{equation*}
	Taking expectation over $\alg$ from both sides, we get
	\begin{equation}\label{eq:72313409}
	\E_{\alg}[\E_{Z, \mc{N}}[x_e \mid f_e]] = \E_{\alg}[f_e].
	\end{equation}
	The left hand side equals $\E_{\alg, Z, \mc{N}}[x_e]$. For the right hand side, by Claim~\ref{cl:frange} we have $\E[f_e] \geq (1-\epsilon)q_e$. 	Replacing both the left hand side and right hand side of (\ref{eq:72313409}) by these bounds, we get
	\begin{equation}
		\E_{\alg, Z, \mc{N}}[x_e] \geq (1-\epsilon) q_e.
	\end{equation}
	Combining this with (\ref{eq:16234421340}) we get
	\begin{equation*}
	\E[x(N')] = \sum_{e \in N'} \E[x_e] \geq (1-\epsilon) \sum_{e \in N'} q_e = (1-\epsilon) q(N'),
	\end{equation*}
	completing the proof.
\end{proof}

We are now ready to prove Lemma~\ref{lem:sizeofx}.

\begin{proof}[Proof of Lemma~\ref{lem:sizeofx}]
	We have
	$$
	\E\Big[\sum_{e}x_e\Big] = \E\Big[\sum_{e \in C} x_e\Big] + \E\Big[\sum_{e \in N} x_e\Big] \stackrel{\text{Claim~\ref{cl:sizeofxcrucial}}}{\geq} q(C) - 31\epsilon \opt + \E\Big[\sum_{e \in N} x_e\Big].
	$$
	Also note that for $e \in N$, $x_e \not= 0$ iff $e \in N'$ by construction of $x$. Thus,
	$$
	\E\Big[\sum_{e \in N} x_e\Big] = 	\E\Big[\sum_{e \in N'} x_e\Big] = \E[x(N')] \stackrel{\text{Claim~\ref{cl:xnpgtqnp}}}{\geq} (1-\epsilon)q(N') \stackrel{\text{Claim~\ref{cl:nplarge}}}{\geq} (1-\epsilon)(q(N)-\epsilon q(C)).
	$$
	Combining the two equations above, we get
	\begin{align*}
		\E\Big[\sum_{e}x_e\Big] &\geq q(C) - 31\epsilon \opt + (1-\epsilon)(q(N)-\epsilon q(C)) > q(C) + q(N) - 33\epsilon \opt\\
		&\stackrel{\text{Lemma~\ref{lem:gap} part (2)}}{\geq} (1-\epsilon)\opt - 33\epsilon \opt \geq (1-34\epsilon)\opt,
	\end{align*}
	concluding the proof.
\end{proof}

==> exptoactualfracmatching.tex <==
\subsection{From the Expected Fractional Matching to an Actual Fractional Matching}\label{sec:turntofracmatching}

We showed that $x$ is an expected fractional matching satisfying $\E[x_v] \leq 1$ for every vertex $v$. However, as mentioned before, there is still a possibility that $x_v > 1$ depending on the coin tosses of the algorithms and the realization. This should never occur in a valid fractional matching. Thus, we define the following scaled fractional matching $y$ based on $x$ which decreases the fractional matching around vertices that deviate significantly from their expectation to 0.

\begin{equation}\label{eq:defy}
	\text{For any edge $e=\{u, v\}$,} \qquad\qquad y_e = \begin{cases}
			x_e/(1+\epsilon) & \text{if $x_v, x_u \leq 1+\epsilon$,}\\
			0 & \text{otherwise.}
	\end{cases}
\end{equation}

\begin{observation}\label{obs:yblossom}
	By definition above, $y$ is a valid fractional matching, i.e. $y_v \leq 1$ for all $v \in V$. In addition, since $y_e \leq x_e$ for all edges $e$, Claim~\ref{cl:xblossom} implies that for all $U \subseteq V$ with $|U| \leq 1/\epsilon$, $y(X) \leq \lfloor \frac{|U|}{2} \rfloor$. That is, $y$ also satisfies all blossom inequalities of size up to $1/\epsilon$.
\end{observation}

It remains to prove that while turning the expected fractional matching $x$ into an actual fractional matching $y$, we don't significantly hurt the matching's size. We address this in the lemma below.

\begin{lemma}\label{lem:ylarge}
	$\E[|y|] \geq (1-55\epsilon)\opt$.
\end{lemma}

The main ingredient in proving Lemma~\ref{lem:ylarge} is the following claim.

\begin{claim}\label{cl:6123719801923}
	For every vertex $v$, $\Pr[x_v > 1+\epsilon] \leq \epsilon^6p$.
\end{claim}

Let us first see how Claim~\ref{cl:6123719801923} suffices to prove Lemma~\ref{lem:ylarge} and then prove it.

\begin{proof}[Proof of Lemma~\ref{lem:ylarge}]
	We have
	\begin{flalign*}
		\sum_{e} y_e &= \sum_{e = \{u, v\}} \mathbbm{1}(x_u \leq 1+\epsilon \text{ and } x_v \leq 1+\epsilon) \frac{x_e}{1+\epsilon} && \text{By definition of $y_e$ in (\ref{eq:defy}).}\\
		&\geq \sum_{e = \{u, v\}} (1-\mathbbm{1}(x_u > 1+\epsilon)-\mathbbm{1}(x_v > 1+\epsilon)) \frac{x_e}{1+\epsilon} && \text{Union bound.}\\
		&= \sum_{e} \frac{x_e}{1+\epsilon} - 2\sum_{v : x_v > 1+\epsilon} \sum_{e \ni v} \frac{x_e}{1+\epsilon} = \sum_{e} \frac{x_e}{1+\epsilon} - 2\sum_{v : x_v > 1+\epsilon} \frac{x_v}{1+\epsilon}.
	\end{flalign*}
	Taking expectation from both sides, we get
	\begin{flalign}
		\nonumber\E\Big[ \sum_e y_e \Big] &\geq \E\Big[\sum_{e} \frac{x_e}{1+\epsilon} - 2\sum_{v : x_v > 1+\epsilon} \frac{x_v}{1+\epsilon}\Big] = \frac{1}{1+\epsilon}\left(\E\Big[\sum_{e} x_e\Big] - 2\E\Big[\sum_{v : x_v > 1+\epsilon} x_v \Big]\right)\\
		\nonumber&\geq \frac{1}{1+\epsilon}\left((1-34\epsilon)\opt - 2\E\Big[\sum_{v : x_v > 1+\epsilon} x_v \Big]\right) \qquad\qquad \text{By Lemma~\ref{lem:sizeofx}.}\\
		\nonumber &\geq (1-35\epsilon)\opt - 2\sum_{v} \Pr[x_v > 1+\epsilon]\E[x_v \mid x_v > 1+\epsilon]\\
		&\geq (1-35\epsilon)\opt - 2\sum_{v} \epsilon^6 p \E[x_v \mid x_v > 1+\epsilon] \qquad\qquad \text{By Claim~\ref{cl:6123719801923}.}\label{eq:98912308}
	\end{flalign}
	We will soon prove that for every vertex $v$, it \underline{deterministically} holds that $x_v \leq \frac{1}{p\epsilon^4}$. Replacing this into the last inequality above, gives the desired bound that
	\begin{flalign*}
		\E\Big[\sum_e y_e \Big] &\geq (1-35\epsilon)\opt - 2\sum_{v} \epsilon^6 p \frac{1}{p \epsilon^4} \geq (1-35\epsilon)\opt - 2\epsilon^2 n \stackrel{\text{Assumption~\ref{ass:optlarge}}}{\geq} (1-35\epsilon)\opt - 20\epsilon \opt \\
		&= (1-55\epsilon)\opt.
	\end{flalign*}
	Now let's see why $x_v \leq \frac{1}{p\epsilon^4}$. Observe from the definition of $x$ that if $v \in V(Z)$ then $x_v \leq 1$ and otherwise
	$$
		x_v = \sum_{e = \{v, u\}} x_e \leq \sum_{e = \{v, u\}} \frac{f_e}{p(1-\Pr[X_u])(1-\Pr[X_v])} \leq \frac{1}{p \epsilon^4} \sum_{e=\{v, u\}} f_e.
	$$
	The last inequality above comes from the fact that for every vertex $w$, $\Pr[X_w] \leq 1-\epsilon^2$ due to Lemma~\ref{lem:independentmatching} part 2, which means $1-\Pr[X_w] \geq \epsilon^2$. 
	
	Now recall from Claim~\ref{cl:frange} part 3 that $\sum_{e \ni v} f_e \leq 1$. Thus we get our desired upper bound that $x_v \leq \frac{1}{p\epsilon^4}$.	 As described above, this completes the proof that $\E[\sum_e y_e] \geq (1-55\epsilon)\opt$.
\end{proof}

We now turn to prove Claim~\ref{cl:6123719801923} that $\Pr[x_v > 1+\epsilon] \leq \epsilon^6 p$ for all $v$.

\newcommand{\eventvz}[0]{\ensuremath{A}}

\begin{proof}[Proof of Claim~\ref{cl:6123719801923}]
	If an edge incident to $v$ belongs to matching $Z$, i.e. if $X_v = 1$ (as defined in Lemma~\ref{lem:independentmatching}), then one can confirm easily from the definition of $x$ in (\ref{eq:crucialxe}) and (\ref{eq:noncrucialxe}) that either $x_v = 1$ or $x_v = 0$, implying that $\Pr[x_v > 1+\epsilon \mid X_v = 1] = 0$. As such, for the rest of the proof, we simply condition on the event that $X_v = 0$.
	
	Similar to the proof of Claim~\ref{cl:expxvlt1} let $u_1, u_2, \ldots, u_r$ be the neighbors of $v$ such that for each $i \in [r]$, (1) edge $e_i = \{v, u_i\}$ is non-crucial, and (2) $d_C(v, u_i) \geq \lambda$. Recall from (\ref{eq:21410238471098412}) that given event $X_v = 0$, it holds that
		\begin{equation*}
			x_v = x_{e_1} + x_{e_2} + \ldots + x_{e_r}.
		\end{equation*}
	
		Let $f'_v := \sum_{i=1}^r f_{e_i}$ and note that $f'_v \leq f_v$ since $f_v$ is sum of $f_e$ of all non-crucial edges $e$ connected to $v$. Claim~\ref{cl:frange} part 4 proves that $\Pr[f_v \geq n_v + 0.1\epsilon] \leq (\epsilon p)^{10}$. Therefore, it also holds that $\Pr[f'_v \geq n_v + 0.1\epsilon] \leq (\epsilon p)^{10}$ since $f'_v \leq f_v$. For the rest of the proof, we regard $f_{e_i}$'s as (adversarially) fixed with the only assumption that $f'_v < n_v + 0.1\epsilon$ which happens with probability at least $1 - (\epsilon p)^{10}$. We denote this event, as well as the event that $X_v = 0$, by $\eventvz$ and prove
		\begin{equation}\label{eq:980989825627}
		\Pr[x_v > 1 + \epsilon \mid \eventvz] \leq 0.5\epsilon^6p,
		\end{equation}
		which clearly is sufficient for proving the claim.
	
		We do this by proving a concentration bound using the second moment method. Consider the variance of $x_v$ conditioned on $\eventvz$:
		\begin{flalign*}
			\Var[x_v \mid \eventvz] = \sum_{i=1}^r \sum_{j=1}^r \Cov(x_{e_i}, x_{e_j} \mid \eventvz).
		\end{flalign*}
		Now that $f_e$'s are fixed, $x_v$ is only a random variable of (1) the randomization used in Lemma~\ref{lem:independentmatching} for obtaining matching $Z$, and (2) the realization of non-crucial edges.
		
		In what follows we identify a condition under which covariance of $x_{e_i}$ and $x_{e_j}$ becomes $0$. We will use this later to upper bound $\Var[x_v \mid \eventvz]$. 
		
		\begin{observation}\label{obs:cov0}
			Let $i, j \in [r]$ be such that $d_C(u_i, u_j) \geq \lambda$. Then $\Cov(x_{e_i}, x_{e_j} \mid \eventvz) = 0$.
		\end{observation}
		\begin{proof}
			We already had $d_C(v, u_i) \geq \lambda$ and $d_C(v, u_j) \geq \lambda$ by definition of $u_i, u_j$. Combined with assumption $d_C(u_i, u_j) \geq \lambda$ and using Lemma~\ref{lem:independentmatching} part 4, we get that $X_v, X_{u_i}, X_{u_j}$ are independent. Realization of $e_i$ and $e_j$ are also independent even given $\eventvz$. This is because these are non-crucial edges and thus are realized independently from $Z$ (according to Lemma~\ref{lem:independentmatching} part 3) or the values of $f$ which are derived from Algorithm~\ref{alg:sampling}.
			
			By definition (\ref{eq:noncrucialxe}), the value of $x_{e_i}$ conditioned on $\eventvz$ is fully determined once we know $X_{u_i}$ and whether $e_i$ is realized. Similarly, the value of $x_{e_j}$ conditioned on $\eventvz$ is fully determined once we know $X_{u_j}$ and whether $e_j$ is realized. These, as discussed above, are independent. Hence $x_{e_i}$ and $x_{e_j}$, conditioned on $\eventvz$, are independent and thus their covariance is 0.
		\end{proof}
		
		Now consider two vertices $u_i$ and $u_j$ (possibly $u_i = u_j$) where $d_C(u_i, u_j) < \lambda$. Here, the covariance may not be 0. But we still can upper bound it as follows:
		\begin{flalign}
		\nonumber \Cov(x_{e_i}x_{e_j} \mid \eventvz) &= \E[x_{e_i}x_{e_j} \mid \eventvz] - \E[x_{e_i} \mid A]\E[x_{e_j} \mid A] \leq \E[x_{e_i}x_{e_j} \mid \eventvz]\\
		\nonumber &\leq \frac{f_{e_i}}{p(1-\Pr[X_v])(1-\Pr[X_{u_i}])} \times \frac{f_{e_j}}{p(1-\Pr[X_v])(1-\Pr[X_{u_j}])}\\
		&\leq \frac{f_{e_i}f_{e_j}}{p^2 \epsilon^8},\label{eq:3819123987}
		\end{flalign}
		where the last inequality follows from Lemma~\ref{lem:independentmatching} part 2 that states for all vertices $w$, $\Pr[X_w] < 1-\epsilon^2$ and thus $1-\Pr[X_w] \geq \epsilon^2$.
		
		Now, for each $i \in [r]$, let $D_i := \{j : d_C(u_i, u_j) < \lambda \}$. Since $C$ is a graph of max degree $\Delta_C$, the $\lambda-1$ neighborhood of each vertex $u_i$ in $C$ includes $\leq (\Delta_C)^{\lambda-1}$ vertices. Thus:
		\begin{equation}\label{eq:87193107123897}
			|D_i| \leq (\Delta_C)^{\lambda-1} \qquad\qquad \text{for every $i \in [r]$.}
		\end{equation}
		Having these, we obtain that
		\begin{flalign*}
			\Var[x_v \mid \eventvz] &= \sum_{i=1}^r \sum_{i=1}^r \Cov(x_{e_i}, x_{e_j} \mid \eventvz) \stackrel{\text{Obs~\ref{obs:cov0}}}{=} \sum_{i = 1}^r \sum_{j \in D_i} \Cov(x_{e_i}, x_{e_j} \mid \eventvz) \stackrel{(\ref{eq:3819123987})}{\leq} \sum_{i = 1}^r \sum_{j \in D_i} \frac{f_{e_i}f_{e_j}}{p^2\epsilon^8} \\
			& = \frac{1}{p^2 \epsilon^8}\sum_{i = 1}^r \Big(f_{e_i}\sum_{j \in D_i} f_{e_j}	\Big) \stackrel{f_{e_j} \leq \frac{1}{\sqrt{\epsilon R}} \text{ by (\ref{eq:deff})}}{\leq} \frac{1}{p^2\epsilon^8} \sum_{i = 1}^r \Big(f_{e_i} |D_i| \frac{1}{\sqrt{\epsilon R}}	\Big)\\
			& \stackrel{(\ref{eq:87193107123897})}{\leq} \frac{(\Delta_C)^{\lambda-1}}{p^2 \epsilon^8\sqrt{\epsilon R}} \sum_{i = 1}^r f_{e_i} \stackrel{\text{Claim~\ref{cl:frange} part 3}}{\leq} \frac{(\Delta_C)^{\lambda-1}}{p^2 \epsilon^8\sqrt{\epsilon R}} \stackrel{\text{Obs~\ref{obs:crucialdegree}}}{\leq} \frac{(1/\tau_+)^{\lambda-1}}{p^2\epsilon^{8.5}\sqrt{R}}.
		\end{flalign*}
		Replacing $R$ with $\frac{1}{2\tau_-}$ and noting that $\tau_- = (1/\tau_+)^{10 g}$, we get that
		\begin{flalign*}
		\Var[x_v \mid A] \leq \frac{2(1/\tau_+)^{\lambda}}{p^2 \epsilon^{8.5}(1/\tau_+)^{10g}} &= \frac{2}{p^2 \epsilon^{8.5}}(\tau_+)^{10g - \lambda}\\
		&< \frac{2\tau_+}{p^2 \epsilon^{8.5}} && \text{By Observation~\ref{obs:ggtlambda} $g \geq \lambda > 1$ and $\tau_+ < 1$.}\\
		&< \frac{2 (\epsilon p)^{50}}{p^2 \epsilon^{8.5}} && \text{Corrolary~\ref{cor:thresholds} part 4.}\\
		&= 2 \epsilon^{41.5} p^{48} < 0.1 \epsilon^8 p.
		\end{flalign*}
		With this upper bound on the variance, we can use Chebyshev's inequality to get
		\begin{equation}\label{eq:cheb18023}
			\Pr\Big[|x_v - \E[x_v \mid \eventvz]| > 0.5\epsilon \,\Big\vert\, \eventvz\Big] \leq \frac{\Var[x_v \mid \eventvz]}{(0.5\epsilon)^2} \leq \frac{0.1 \epsilon^8 p}{0.25 \epsilon^2} < 0.5\epsilon^6 p.
		\end{equation}
		Next, recall from (\ref{eq:421610986201363}) in the proof of Claim~\ref{cl:expxvlt1} that $\E[x_v \mid v\not\in V(Z)] \leq \frac{\sum_{i=1}^r \E[f_{e_i}]}{1-\Pr[X_v]} = \frac{f'_v}{1-\Pr[X_v]}$. Event $\eventvz$ in addition to $v \not\in V(Z)$ also fixes the value of $f'_v$. But recall that event $\eventvz$ (as we defined it) guarantees $f'_v \leq n_v + 0.5\epsilon$. Therefore, we get
		\begin{equation}\label{eq:74777748123}
			\E[x_v \mid \eventvz] \leq \frac{n_v + 0.5\epsilon}{1-\Pr[X_v]} \stackrel{\Pr[X_v] < c_v}{\leq} \frac{n_v + 0.5\epsilon}{1-c_v} \stackrel{n_v \leq 1-c_v}{\leq} \frac{1-c_v+0.5\epsilon}{1-c_v} \leq 1 + 0.5\epsilon.
		\end{equation}
		Combining (\ref{eq:cheb18023}) and (\ref{eq:74777748123}) we get the claimed inequality of (\ref{eq:980989825627}) that 
		$$
		\Pr[x_v > 1+\epsilon \mid \eventvz] \leq \Pr[|x_v - \E[x_v \mid A]| > 0.5\epsilon \mid \eventvz] \leq 0.5\epsilon^6p,
		$$
		which as described before suffices to prove $\Pr[x_v > 1+\epsilon] \leq \epsilon^6p$.
\end{proof}




==> ind-algorithm.tex <==


We say $P = ((\mc{C}_0, M_0), \ldots, (\mc{C}_\alpha, M_\alpha))$ is a {\em profile} if each $\mc{C}_i$ is a subgraph of $C$ and each $M_i$ is a matching of $\mc{C}_i$. Furthermore, we call a sequence $W = ((e_1, s_1), \ldots, (e_k, s_k))$ a {\em hyperwalk} of size $k$ if the following conditions hold:
\begin{enumerate}[itemsep=0pt,topsep=5pt]
	\item Each $s_i$ is an integer in $\{0, \ldots, \alpha\}$.
	\item Each $e_i$ is an edge in graph $C$ and sequence $(e_1, e_2, \ldots, e_k)$ is a walk in graph $C$.
\end{enumerate}
We say $P\Delta W := ((\mc{C}_0, M'_0), \ldots, (\mc{C}_\alpha, M'_\alpha))$ is the result of {\em applying} $W$ on $P$ if:
$$
	M'_i = M_i \cup \{ e_j \mid j \text{ is odd, and } s_j = i\} \setminus \{ e_j \mid j \text{ is even, and } s_j = i\}, \qquad \text{for all $i \in \{0, \ldots, \alpha\}$}.
$$
\begin{definition}[Augmenting hyperwalks] \label{def:aug}
For every vertex $v$, let $d_P(v) := \big |\{ i \mid v \in V(M_i) \}\big |$. We say $W$ is an {\em augmenting-hyperwalk} of $P$ if it satisfies the three following conditions.
\begin{enumerate}[itemsep=0pt,topsep=5pt]
	\item $P \Delta W$ is a profile, i.e. each  $M'_i$ in $P \Delta W$ is a matching of graph $\mc{C}_i$.
	\item For all vertices $v$ in walk $(e_1, \ldots, e_k)$ except its first and last vertex, $d_P(v) = d_{P\Delta W}(v)$. 
	\item For the first and last vertices $v$ in walk $(e_1, \ldots, e_k)$, $d_P(v) + 1 = d_{P \Delta W}(v)$.
\end{enumerate}
\end{definition}
Having defined augmenting-hyperwalks, we can now formally state the algorithm---see Algorithm~\ref{alg:crucial}. The algorithm is recursive. Given a realization $\mc{C}$ of $C$, algorithm $\findmatching{r}{\mc{C}}$ uses algorithm $\findmatching{r-1}{\mc{C}}$ as a subroutine and then returns a matching of $\mc{C}$. The base algorithm $\findmatching{0}{\mc{C}}$ returns an empty matching. We will show that for $t = 1/\epsilon^5$, algorithm $\findmatching{t}{\mc{C}}$ satisfies the properties of Lemma~\ref{lem:independentmatching}. 



\begin{tboxalgh}{\findmatching{r}{\mc{C}}}\label{alg:crucial}
	\vspace{-0.3cm}
	\begin{enumerate}[label=(\arabic*), itemsep=-2pt, leftmargin=23pt]
		\item If $r = 0$, return $\emptyset$.
		\item Draw $\alpha := 1/\epsilon^3-1$ realizations $\mc{C}_1, \ldots, \mc{C}_\alpha$ of $C$  where each realization $\mc{C}_{i}$ includes each edge $e$ of $C$ independently with probability $p_e$. Also let $\mc{C}_0 := \mc{C}$.
		\item Consider profile $P = ((\mc{C}_0, M_0), \ldots, (\mc{C}_\alpha, M_\alpha))$ where $M_i = \findmatching{r-1}{\mc{C}_i}$.
		\item For every vertex $v$, define $\gamma_{v, r-1} := \Pr[\text{$v$ is matched in \findmatching{r-1}{\mc{C}'}}]$ where the probability is taken over a random realization $\mc{C}'$ of $C$ and the randomization of the algorithm. 
		\item If $\gamma_{v,r-1} < c_v-2\epsilon^2$ call vertex $v$ {\em unsaturated} and {\em saturated} otherwise. 
		\item Construct a graph $H=(V_H, E_H)$ as described next. For every possible augmenting-hypewalk of size smaller than $2/\epsilon$ from $P$, we put a vertex in $V_H$ iff the first and last vertices in the walk are unsaturated. Moreover, we put an edge in $E_H$ between two nodes $u, v \in V_H$ iff their corresponding walks share at least a vertex.
		\item  \label{line:setI}$I \gets \apxMIS{H, \epsilon}$. \algcomment{This is an algorithm that returns an independent set of expected size at least $1-\epsilon$ fraction of some maximal independent set (MIS) of $H$.}
		\item $P' \gets P$.
		\item Iterate over all augmenting-hyperwalks $W \in I$ and apply them, i.e. set $P' \gets P' \Delta W$.
	\item Let $P'=((\mc{C}_0, M'_0), \ldots, (\mc{C}_\alpha, M'_\alpha))$ be the final profile. Return matching $M'_0$.
	\end{enumerate}
\end{tboxalgh}
We note a useful observation that essentially implies the entries of profile $P'$, which can be thought of as random variables of realization $\mc{C}$ and randomizations of the algorithm, are all drawn from the same distribution. The proof is essentially based on the fact that matchings $M_0, \ldots, M_\alpha$ are all drawn from the same distribution and treated symmetrically in algorithm, thus the resulting matchings $M'_0, \ldots, M'_\alpha$ all have the same distribution. See Section~\ref{sec:proofs} for a more formal proof.

\begin{observation}\label{obs:samedist}
	Matchings $M'_0, \ldots, M'_\alpha$ in profile $P'$ of algorithm $\findmatching{r}{\mc{C}}$ for any $r$ have the same distribution. That is, for any $i, j \in \{0, \ldots, \alpha\}$ and any matching $M'$ of $G$, $\Pr[M'_i = M'] = \Pr[M'_j = M']$.
\end{observation}

The algorithm operates only on the crucial edges and is thus clearly independent of the non-crucial edges and their realizations. Therefore, property 3 of Lemma~\ref{lem:independentmatching} is automatically satisfied. In what follows, we prove the other 3 properties in Sections~\ref{sec:p1}, \ref{sec:p2}, and \ref{sec:p4}.

\subsection{Lemma~\ref{lem:independentmatching} Property 1: The Matching's Size}\label{sec:p1}
\input{matchingsize}


\subsection{Lemma~\ref{lem:independentmatching} Property 2: Matching Probabilities}\label{sec:p2}
\input{matchingprobs}

\subsection{Lemma~\ref{lem:independentmatching} Property 4: Matching Independence}\label{sec:p4}
\input{matchingindependence}

%We define $F$ with the set of vertices $V$ to be a colorful multi-graph that contains an edge $e$ with color $i\in [0, \alpha]$ for any edge $e\in \mc{C}_i$. We also define $M^F$ a subgraph of $F$, to have an edge $e$ with color $i$ iff $e\in M_i$. Observe that coloring of edges in $M^\Psi$ is a valid edge coloring since it is a union of a set of matchings with different colors. We are interested to find a walk in graph $\Psi$ and flip the membership of its edges in graph $M^\Psi$ to increases its size while it still has a valid edge coloring. For the purpose that this procedure will be used, we need to make sure that this change does not increase the degree of saturated vertices in $M^F$. We call an augmenting walk any walk in graph $F$ that satisfies these properties 
%
% Let $\mc{S}^F$ denote the set of all subgraphs of $F$ that satisfy the mentioned properties. To increase size of $M^F$ in few iterations, we want to find a subset of vertex disjoint trails in $\mc{S}^\Psi$ and flip the membership of all their edges in $M^\Psi$ in a single iteration. To achieve this, we use the random greedy MIS algorithm on a graph that has a vertex for any element of $\mc{S}^\Psi$ and an edge between any two of them that are not vertex disjoint. The gives us a set of vertex disjoint walks



%\begin{definition}[Augmenting trail] Given $\alpha+1$ subgraphs $\mc{C}_{0}, \dots, \mc{C}_{\alpha}$  of a graph $C$ and a matching for any of them $M_{0}, \dots, M_{\alpha}$, 
%\\
%For any walk $e_1, \dots, e_l$ of length $l$ in graph $C$, and a sequence of colors $c_1, \dots, c_l$ where $c_i\in[0,\dots, \alpha]$ we say $(e_1, c_1)\dots (e_l, c_l)$ is a an alternating trail iff
%\begin{itemize}
%\item for any color $i\in [l]$ graph $\mc{C}_{k_i}$ contains edge $e_i$, and
%\item for any consecutive elements  $(e_i, k_i)$ and $(e_j, k_j)$, either  $e_i \in M_{k_i}$ or $e_j \in M_{k_j}$. 
%\end{itemize}
%
%for any consecutive $i, j \in [l]$, graph $\mc{C}_{k_i}$ contains edge $(v_i, u_i)$,   and either $(v_i, u_i) \in M_{k_i}$ or $(v_j, u_j) \in M_{k_j}$. Further, any alternating path is an augmenting trail, iff $v_1$ and $v_l$
%\end{definition}

%
%Let $H$ be the subgraph of $G$ including only its crucial edges and let $H_p$ be the realized subgraph of $H$. Similar to the notation used in Lemma~\ref{lem:independentmatching} we let $\Delta$ be the maximum degree in graph $H$.
%
%Property (1) of Lemma~\ref{lem:independentmatching} ensures that the 
%
%
%implies roughly speaking that $c'_v$ has to be close to $c_v$ for almost every vertex $v$. The main challenge is to satisfy this property, while also ensuring the independence property (i.e. property 2 of Lemma~\ref{lem:independentmatching}).
%
%%\vspace{2cm}
%
%To do this, we assume that the algorithm has access to an  infinite tape \b{r} of random bits and each node of the graph $G$ has a unique ID in $\{1, \ldots, n\}$. Having these, the algorithm has to construct a matching $M$ of graph $G_p$. Instead of $M$, we may write $M(G_p, \b{r})$ to emphasize that the only sources of randomization for determining matching $M$ are the realization $G_p$ and the tape \b{r}.
%
%We measure the efficiency of an algorithm by the concept of verifiers. Formally, a verifier has no knowledge of graph $G_p$ or even $G$, but given the random tape \b{r}, for any given vertex $v$ has to determine whether $v$ is matched in $M(G_p, \b{r})$ by conducting the following queries:
%\begin{enumerate}
%	\item \neighbors{u}: This query returns all neighbors of vertex $u$ in graph $G$ (note that this is the original graph $G$ not the realized graph $G_p$).
%	\item \isrealized{e}: This query returns whether a given edge $e$ in graph $G$ is realized in graph $G_p$.
%\end{enumerate}
%
%%We note that the definition above is close to that of Local Computation Algorithms (LCA's), but has two crucial differences. First, the graph under consideration is stochastic. Second, we assume that the algorithm has access to an infinite random tape.
%
%Define $\dependent(v, \b{r}, G_p)$ to be the set of vertices and edges on which the verifier conducts the queries above in answering whether $v$ is matched in $M(G_p, \b{r})$. Moreover, define 
%\begin{equation}
%	\dependent(v) := \{x \mid \exists G_p, \b{r} \text{ such that } x \in \dependent(v, \b{r}, G_p) \},
%\end{equation}
%which is the set of vertices/edges that may be queried for some tape $\b{r}$ and some realization $G_p$.

%\vspace{3cm}

%To do this, we operate in the following model of computation. The algorithm has access to an infinite tape \b{r} of random bits and each node of the graph $G$ has a unique ID in $\{1, \ldots, n\}$. The algorithm can conduct queries of two forms: 
%\begin{enumerate}
%	\item \neighbors{v}: This query returns all neighbors of vertex $v$ in graph $G$ (note that this is the original graph $G$ not the realized graph $G_p$).
%	\item \isrealized{e}: This query returns whether a given edge $e$ in graph $G$ is realized in graph $G_p$.
%\end{enumerate}
%
%Now, given any edge $e$, the algorithm has to return whether $e$ belongs to the matching $M$. These responses for different edges should be consistent with each other if the same random seed \b{r} and realization are used. That is, they should form a valid matching $M$ of $G_p$.
%
%\vspace{2cm}
%Some sketches before I start writing:
%\begin{enumerate}
%	\item Let's use $A_i(\b{r}, C_p)$ to denote the outcome of the algorithm (which is a matching) after $i$ phases and when $\b{r}$ denotes the set of random tapes on the edges used throughout the algorithm and $C_p$ denotes the realized crucial edges.
%	\item Define $A_0(\b{r}, C_p) = \emptyset$.
%	\item To determine matching $A_i(\b{r}, C_p)$:
%	\begin{enumerate}
%		\item For $\eta = 1/\epsilon$, construct $\eta + 1$ independent random tapes $\b{r}^{(0)}, \b{r}^{(1)}, \ldots, \b{r}^{(\eta)}$ and $\eta$ independent random realizations $C_p^{(1)}, \ldots, C_p^{(\eta)}$. We derive all of these from the randomization available in $\b{r}$.
%		\item Consider matching $A_0 = A_{i-1}(\b{r}^{(0)}, C_p)$ and matchings $A_1 = A_{i-1}(\b{r}^{(1)}, C_p^{(1)}), \ldots, A_\eta = A_{i-1}(\b{r}^{(\eta)}, C_p^{(\eta)})$.
%		\item Find augmenting paths of small size passing through these matchings and apply them obtaining matchings $A'_0, A'_1, \ldots, A'_\eta$.
%		\item Return $A'_0$.
%	\end{enumerate}
%\end{enumerate}

==> ind-intuitions.tex <==

In this section, we give an overview of our algorithm for proving Lemma~\ref{lem:independentmatching}. We emphasize that the overview given here is deliberately informal to describe the main intuitions, with the hope that it makes the algorithm and its analysis more accessible.

Satisfying property~3 required by Lemma~\ref{lem:independentmatching} turns out to be easy. Recall that we are constructing matching $Z$ on the realized {\em crucial} edges, thus we can simply ignore realization of non-crucial edges and automatically satisfy property~3. Among the other 3, let us first focus on property~4. How can we argue that the output matching satisfies the required independence property? We show that the \local{} model of computation can be naturally used for this purpose. We start with the formal definition of the model and then describe how it can be used in this case.

\smparagraph{The \local{} model \cite{DBLP:journals/siamcomp/Linial92}.} In the \local{} model, the input is a graph and there is a processor on each node of this graph. Computation proceeds in synchronous rounds and in each round, each processor can send a message (of any size) to each of its neighbors. The goal is to output a property of this communication graph, e.g. a matching of it. At the end, each node should know its part of the output, e.g. which one of its edges, if any, is part of the matching.


\smparagraph{Why the \local{} model.} A particularly useful property of any $r$-round \local{} algorithm is that the output of each node essentially depends only on its $r$-hop neighborhood. That is, having the $r$-hop neighborhood of each node $v$ (including the random tapes of the nodes in the neighborhood), we can uniquely determine the output of $v$. Therefore if the shortest path between two nodes is at least $2r+1$, their outputs are essentially independent of each other after $r$ rounds. 

This is how we prove property~4 of Lemma~\ref{lem:independentmatching} is satisfied: We give a \local{} algorithm operating on graph $C$ where each vertex is initially only aware of the realization of its incident edges. We show that the algorithm within $< \lambda/2$ rounds, finds a matching satisfying the other 3 properties. Then property~4 will be automatically satisfied. That is, for every subset $I$ of the vertices with pairwise distance at least $\lambda$, their outputs will be independent.

\smparagraph{Overview of the algorithm.} The challenge is to ensure that the algorithm has low round-complexity while also satisfying properties 1 and 2. That is, the reported matching $Z$ should be large in expectation (property 1), and that no vertex $v$ should be matched with a larger probability than that specified in property~2. If one ignores the 2nd property, then simply finding a $(1-\epsilon)$-approximate maximum matching in graph $\mc{C}$ will satisfy the first property. And we remark that $O(\log \Delta_C)$-round algorithms (with no dependence on $n$) do exist for this purpose. However, bounding at the same time, the probability that each vertex is matched complicates things. 

Our general idea for the algorithm is as follows: We define a recursive algorithm $\findmatching{r}{\mc{C}}$ (Algorithm~\ref{alg:crucial}) which uses $\findmatching{r-1}{\mc{C}}$ as a subroutine. The base algorithm $\findmatching{0}{\mc{C}}$ returns an empty matching. Let us use $Z_r$ to denote the matching returned by $\findmatching{r}{\mc{C}}$. It will hold that
$$
0 = \E[|Z_0|] \leq \E[|Z_1|] \leq \E[|Z_2|] \leq \ldots 
$$
until eventually for large enough $t = O_\epsilon(1)$, $\E[|Z_t|]$ is desirably large, satisfying property~1. At the same time, we will ensure that for any vertex $v$, the probability that it gets matched in $Z_r$ never exceeds the upper bound of property~2 for any $r$. 

Suppose that for a vertex $v$, we hit this upper bound on the probability that it is matched for algorithm $\findmatching{r}{\mc{C}}$. At this point, we will mark $v$ as {\em saturated} and ensure that we never increase the probability of it being matched. But to keep increasing the matching's size, it may be necessary to say remove a matching edge $\{v_1, v_2\}$ between two saturated vertices $v_1$ and $v_2$, so that we can add two edges $\{v_1, v_3\}$ and $\{v_2, v_4\}$ to the matching where $v_3$ and $v_4$ are unsaturated. Such structures are similar to augmenting paths. However, since the graph is stochastic, these edges $\{v_1, v_2\}, \{v_1, v_3\}, \{v_2, v_4\}$ may not necessarily be part of one realization. We call these natural generalizations of augmenting paths, ``augmenting hyperwalks'' (see Section~\ref{sec:formalcrucialalg}) and show that they can be used to increase the matching size while not increasing probability of saturated vertices getting matched.

In Section~\ref{sec:formalcrucialalg} we present a centralized view of the algorithm. In Section~\ref{sec:p1} we analyze the expected size of the matching returned by this algorithm and argue that it satisfies property~1 of Lemma~\ref{lem:independentmatching}. In Section~\ref{sec:p2} we prove the upper bound on the probability of each vertex getting matched, thereby proving property~2 of Lemma~\ref{lem:independentmatching}. Finally, in Section~\ref{sec:p4} we show that the algorithm has an efficient \local{} implementation, satisfying property~4 of Lemma~\ref{lem:independentmatching}.





==> matchingindependence.tex <==
In this section, we prove that algorithm $\findmatching{t}{\mc{C}}$ satisfies property 4 of Lemma~\ref{lem:independentmatching}. That is, for every subset $I= \{v_1, \ldots, v_k\}$ of the vertices such that $d_C(v_i, v_j) \geq \lambda$ for all $v_i, v_j \in I$, random variables $X_{v_1}, \ldots, X_{v_k}$ are independent. Recall that $X_v$ for a vertex $v$ is the indicator of the event that $v$ is matched in the matching returned by \findmatching{t}{\mc{C}}. We also, again, emphasize that this ``independence'' is with regards to the randomization of realization $\mc{C}$ of $C$ on which $Z$ is constructed, and the randomization of algorithm $\findmatching{t}{\mc{C}}$ itself.

In Section~\ref{sec:crucialoverview} we gave an overview of how we can argue about such independence via an implementation of the algorithm in the \local{} model of computation. Here we give this implementation.


\smparagraph{Initialization.} The communication network is graph $C$. Each node $v$ is initially given the following information: Its incident edges in $C$ and how they are realized, the maximum degree $\Delta_C$ of graph $C$, parameter $\epsilon$, and the value of $c_v$. Note that to gather information about realization of edges further away, the nodes need to communicate. Also note that even though the value of $c_v$ may reveal some information about graph $G$ (or $C$), it crucially reveals no information about the realization $\mc{C}$ of $C$, or other sources of randomization used by the algorithm. Thus, property 4 can still be satisfied if we manage to show the algorithm can be implemented in few rounds of this model.

\smparagraph{The \apxMIS{H, \epsilon} algorithm.} First, we mention that subroutine \apxMIS{H, \epsilon} already has an efficient \local{} implementation whose round-complexity depends only on the maximum degree of $H$ and $\epsilon$, without essentially any dependence on the number of nodes in $H$. Any implementation with such round-complexity can be used in our case. For instance, we use one implied in \cite{DBLP:conf/soda/Ghaffari19} (see Appendix~\ref{app:weakmis} for details):

\begin{lemma}[\cite{DBLP:conf/soda/Ghaffari19}]\label{lem:apxMIS}
	Given a graph $H$ of max degree $\Delta$ and any parameter $\epsilon$, there is a \local{} algorithm $\apxMIS{H, \epsilon}$ that returns an independent set $I$ of $H$ in $O(\log \frac{\Delta}{\epsilon})$ rounds such that the expected size of $I$ is at least $(1-\epsilon)$ fraction of some maximal independent set of $H$.
\end{lemma}

We give a \local{} implementation of Algorithm~\ref{alg:crucial} which proves the following:

\begin{claim}\label{cl:localimp}
	For any $r \geq 0$, algorithm $\findmatching{r}{\cdot}$ can be implemented in $O(r \epsilon^{-4}\log{\Delta_C})$ rounds of \local{}.
\end{claim}

\begin{proof}
We prove the claim by induction on $r$. For the base case, algorithm \findmatching{0}{\cdot} can be implemented in 0 rounds since the output is always the empty matching. We assume that algorithm \findmatching{r-1}{\cdot} can be implemented in $\beta(r-1)\epsilon^{-4}\log \Delta_C$ rounds where $\beta > 1$ is a sufficiently large absolute constant that we fix later, and prove that $\findmatching{r}{\cdot}$ can be implemented in $\beta r\epsilon^{-4}\log \Delta_C$ rounds. 

\textbf{Step 1.} First, the algorithm draws $\alpha$ realizations $\mc{C}_1, \ldots, \mc{C}_\alpha$. Since information about realization of edges is stored locally on their incident vertices, we can easily generate these random realizations in $O(1)$ rounds. After that, on each graph $\mc{C}_i$ for $i \in \{0, \ldots, \alpha\}$, we recursively run the $(\beta(r-1)\epsilon^{-4}\log \Delta_C)$-round implementation of $\findmatching{r-1}{\mc{C}_i}$. Note that all of these can run in parallel. The overall round-complexity of this step, is thus $\beta(r-1)\epsilon^{-4}\log \Delta_C + O(1)$.

\textbf{Step 2.} Next, we need to compute $\gamma_{v, r-1}$ for each vertex $v$, which recall is the probability that $v$ is matched in $\findmatching{r-1}{\mc{C'}}$ where $\mc{C}'$ is a random realization of $C$. The crucial observation here is that since $\findmatching{r-1}{\cdot}$ can, by the induction hypothesis, be implemented within only $\beta(r-1)\epsilon^{-4}\log \Delta_C$ rounds, $\gamma_{v, r-1}$ is merely a function of the topology induced in the $(\beta(r-1)\epsilon^{-4}\log \Delta_C)$-hop of $v$. We first gather this neighborhood of $v$, which can be done in $(\beta(r-1)\epsilon^{-4}\log \Delta_C)$ rounds, then compute $\gamma_{v, r-1}$. We note that this gathering part can be done in parallel to the operations of Step 1. Therefore, overall, Steps 1 and 2 take $(\beta(r-1)\epsilon^{-4}\log \Delta_C + O(1))$ rounds. Having $\gamma_{v, r-1}$ for each vertex $v$, we can then determine for each vertex whether it is saturated or unsaturated since we are given the value of $c_v$ in the initialization step. 

\textbf{Step 3.} The next step is constructing graph $H$. In graph $H$, each vertex corresponds to a walk of size at most $2/\epsilon$ in $C$. Therefore, each vertex in $C$ can first gather all such walks around it in $O(1/\epsilon)$ rounds, and then determine which one of them are augmenting-hyperwalks satisfying the required properties to be considered as a node of $H$. Determining the edges of $H$ can also be done locally; once we construct the vertices, there will be an edge between any two walks that share a vertex. Therefore, overall, graph $H$ can be constructed in $O(1/\epsilon)$ rounds.

\textbf{Step 4.} Once we construct $H$, we run the \local{} implementation of $\apxMIS{H, \epsilon}$ mentioned in Lemma~\ref{lem:apxMIS} on graph $H$. We emphasize that our communication network here is graph $C$, not $H$. However, any message between two nodes of $H$ can be sent over network $C$ within $O(1/\epsilon)$ rounds. This is because any two incident nodes of $H$, are walks of size at most $O(1/\epsilon)$ in $C$ that share at least a vertex. The overall running time of this procedure is thus  $O(\frac{1}{\epsilon} \times \log \frac{\Delta_H}{\epsilon})$. We note that $\Delta_H = O(\epsilon^{-1} ((\alpha+1)\Delta_C)^{2/\epsilon})$. To see this, fix any walk $w$ with a corresponding node in $H$. This walk has at most $2/\epsilon$ nodes in $C$. Now each node in $C$ is incident to $O(((\alpha+1)\Delta_C)^{2/\epsilon})$ hyperwalks: There are $O((\Delta_C)^{2/\epsilon})$ walks of size $\leq 2/\epsilon$ branching out of each of the nodes, and each edge of the walk can take on $\alpha+1$ labels from $\{0, \ldots, \alpha\}$ to be transformed to a hyperwalk. Therefore, overall the number of rounds required for this part of the algorithm is
$$
	O\left(\frac{1}{\epsilon} \times \log \frac{\Delta_H}{\epsilon}\right) = O\left(\frac{1}{\epsilon} \log \frac{\epsilon^{-1} ((\alpha+1)\Delta_C)^{2/\epsilon}}{\epsilon} \right) = O\left(\epsilon^{-4} \log \Delta_C \right),
$$
where the last equality comes from the fact that $\alpha = \poly(\epsilon^{-1})$.

\textbf{Step 5.} Finally, applying the augmenting-hyperwalks chosen in $I$ is simple and can be done in $O(1/\epsilon)$ rounds since these walks are of size $\leq 2/\epsilon$.

\textbf{Round-complexity.} Let $\beta_2$ be a sufficiently large constant by multiplying which we can surpass the $O$-notations. We get
\begin{flalign*}
\text{\# of rounds} &\leq 
\underbrace{\beta(r-1)\epsilon^{-4}\log \Delta_C + \beta_2}_{\text{Steps 1 and 2}} + \underbrace{\beta_2(1/\epsilon)}_{\text{Step 3}} + \underbrace{\beta_2(\epsilon^{-4}\log\Delta_C)}_{\text{Step 4}} + \underbrace{\beta_2(1/\epsilon)}_{\text{Step 5}}\\
 &< \beta(r-1)\epsilon^{-4}\log \Delta_C + 4\beta_2(\epsilon^{-4}\log\Delta_C)\\
	&= \Big( \beta(r-1)+4\beta_2 \Big)\epsilon^{-4}\log\Delta_C.
\end{flalign*}
Since $\beta_2$ is an absolute constant that does not depend on $\beta$, we can set $\beta$ to be large enough with respect to it. Setting $\beta = 4\beta_2$ is sufficient since
$$
	\Big( \beta(r-1)+4\beta_2 \Big)\epsilon^{-4}\log\Delta_C = \beta r \epsilon^{-4}\log \Delta_C.
$$
This concludes the proof of the induction step, and consequently the proof of Claim~\ref{cl:localimp}.
\end{proof}

We showed in Claim~\ref{cl:localimp} that algorithm \findmatching{r}{\mc{C}}, for any $r$, can be implemented within $O(r\epsilon^{-4}\log \Delta_C)$ rounds of \local{}. Our final algorithm for Lemma~\ref{lem:independentmatching} is $\findmatching{t}{\mc{C}}$ where we set $t = 1/\epsilon^5$. Thus, the output of each vertex can be determined within $\lambda'=O(\epsilon^{-9}\log\Delta_C)$ rounds. This, as described, proves property 4 of Lemma~\ref{lem:independentmatching} since $\lambda=\epsilon^{-10}\log \Delta_C$ is larger than $\lambda'/2$ given that $\epsilon$ is small enough to surpass the hidden constants in the $O$-notation. (Recall that we can assume $\epsilon$ is smaller than any needed constant.)







==> matchingprobs.tex <==
In this section, we prove that algorithm $\findmatching{t}{\mc{C}}$ satisfies property 2 of Lemma~\ref{lem:independentmatching} that for each vertex $v$, $\Pr[X_v] \leq \max\{c_v - \epsilon^2, 0\}$. Recall that $X_v$, as defined in Lemma~\ref{lem:independentmatching}, is the indicator of the event that $v$ is matched in \findmatching{t}{\mc{C}}, and the probability is taken over both the realization $\mc{C}$ and the randomization of algorithm $\findmatching{t}{\mc{C}}$.

Let us use $X_{v, r}$ to denote the event that vertex $v$ gets matched in matching $\findmatching{r}{\mc{C}}$. It holds that $X_{v, t} = X_v$. Therefore, it suffices to show that $\Pr[X_{v, t}] \leq \max\{c_v - \epsilon^2, 0\}$. We will, however, prove a stronger claim:

\begin{claim}\label{cl:p2holds}
	For every integer $r$ and for every vertex $v$, it holds that $\Pr[X_{v, r}] \leq \max\{c_v - \epsilon^2, 0\}$.
\end{claim}

We prove this by indiction on $r$. For the base case $r=0$, algorithm $\findmatching{0}{\mc{C}}$ returns an empty matching $\emptyset$. Therefore $\Pr[X_{v, 0}] = 0$ for all vertices $v$, clearly satisfying the claim. For the induction step, fix any vertex $v$. We suppose that $\Pr[X_{v, r-1}] \leq \max\{c_v - \epsilon^2, 0\}$ and prove that it continues to hold that $\Pr[X_{v, r}] \leq \max\{c_v - \epsilon^2, 0\}$. We start with a definition.

\begin{definition}
Define $\rho_v$ to be the fraction of matchings $M_0, \ldots, M_\alpha$ in which $v$ is matched and define $\rho'_v$ similarly with respect to matchings $M'_0, \ldots, M'_\alpha$. More precisely,
$$
	\rho_v := \frac{|\{i : v \in V(M_i) \}|}{\alpha + 1}, \qquad \text{ and } \qquad \rho'_v := \frac{|\{i : v \in V(M'_i) \}|}{\alpha + 1}.
$$	
\end{definition}


\begin{observation}
	$\E[\rho_v] = \Pr[X_{v, r-1}]$ and $\E[\rho'_v] = \Pr[X_{v, r}]$.
	%We emphasize that the expectations and probabilities are taken over both the randomization of realizations $\mc{C} = \mc{C}_0, \mc{C}_1, \ldots, \mc{C}_\alpha$ and the randomizations used in obtaining matchings $M_0, \ldots, M_\alpha$ and $M'_0, \ldots, M'_\alpha$.
\end{observation}
\begin{proof}
	For any $i \in \{0, \ldots, \alpha\}$, we have $\Pr[v \in V(M_i)] = \Pr[X_{v, r-1}]$ since $M_i = \findmatching{r-1}{\mc{C}_i}$ and $\mc{C}_i$ is picked from the same distribution that the actual realization $\mc{C}$ is picked from. Thus: 
	$$
		\E[\rho_v] = \E\left[\frac{\sum_{i=0}^\alpha \mathbbm{1}(v \in V(M_i))}{\alpha+1}\right] = \frac{1}{\alpha+1} \sum_{i=0}^\alpha \Pr[v \in V(M_i)] = \frac{1}{\alpha+1} \sum_{i=0}^\alpha \Pr[X_{v, r-1}] = \Pr[X_{v, r-1}].
	$$
	For the second equality, first observe that since $M'_0$ is the matching returned by $\findmatching{r}{\mc{C}}$, then $X_{v, r}$ is by definition exactly the event that $v \in V(M'_0)$ and thus $\Pr[X_{v, r}] = \Pr[v \in V(M'_0)]$. Moreover, due to symmetry of the algorithm in constructing $M'_0, \ldots, M'_\alpha$, it holds for any $i \in [\alpha]$ that $\Pr[v \in V(M'_i)] = \Pr[v \in V(M'_0)] = \Pr[X_{v, r}]$. Therefore, we get:
	$$
		\E[\rho'_v] = \E\left[\frac{\sum_{i=0}^\alpha \mathbbm{1}(v \in V(M'_i))}{\alpha+1}\right] = \frac{1}{\alpha+1} \sum_{i=0}^\alpha \Pr[v \in V(M'_i)] = \frac{1}{\alpha+1} \sum_{i=0}^\alpha \Pr[X_{v, r}] = \Pr[X_{v, r}],
	$$
	concluding the proof.
\end{proof}

In algorithm \findmatching{r}{\mc{C}}, we mark $v$ as either saturated or unsaturated depending on the value of $\gamma_{v, r-1}$. Note from definition of $\gamma_{v, r-1}$ that $\gamma_{v, r-1} = \Pr[X_{v, r-1}]$. Therefore, $v$ is marked as saturated if $\Pr[X_{v, r-1}] \geq c_v - 2\epsilon^2$ and unsaturated if $\Pr[X_{v, r-1}] < c_v - 2\epsilon^2$. We consider the two cases individually.

\smparagraph{If $v$ is saturated.} In this case, by definition of graph $H$, vertex $v$ cannot start or end any augmenting-hyperwalk with a corresponding vertex in $H$ (and for that matter in $I$). By definition of augmenting-hyperwalks, for all vertices (except the endpoints of the walk) applying the hyperwalk does not change the number of matchings in which the vertex is part of. Therefore, if $v$ is saturated, $\rho_v = \rho'_v$ and thus $\Pr[X_{v, r}] = \Pr[X_{v, r-1}] \leq \max\{c_v - \epsilon^2, 0\}$ where the latter inequality comes from the induction's hypothesis.

\smparagraph{If $v$ is unsaturated.} Note that in graph $H$ by definition we have edges between any pair of augmenting-hyperwalks that share a vertex in the graph. Therefore, the independent set $I$ of $H$ can include at most one augmenting-hyperwalk $W$ that includes vertex $v$. If $v$ is not an end-point of $W$, then as in the case above, we get $\rho_v = \rho'_v$. However, if $v$ is an end-point of $W$, then by definition of augmenting-hyperwalks, there will be one (and only one) $i$ where $v \in V(M'_i)$ and $v \not\in V(M_i)$. In this case, we get that
$$
	\rho'_v = \frac{|\{i : v \in V(M'_i) \}|}{\alpha + 1} = \frac{|\{i : v \in V(M_i) \}| + 1}{\alpha + 1} = \rho_v + \frac{1}{\alpha+1} \stackrel{\alpha = 1/\epsilon^3-1}{<} \rho_v + \epsilon^2.
$$
Since in this case, we had $\rho_v < c_v - 2\epsilon^2$, we get $\rho'_v < c_v - 2\epsilon^2 + \epsilon^2 = c_v -\epsilon^2$. Therefore the induction's hypothesis still holds that $\Pr[X_{v, r}] < \max\{c_v - \epsilon^2, 0\}$, completing the proof of Claim~\ref{cl:p2holds}.




==> matchingsize.tex <==
In this section, we prove that algorithm $\findmatching{t}{\mc{C}}$  satisfies the first property of Lemma~\ref{lem:independentmatching}. That is the matching $Z$ returned by this algorithm satisfies $\E[|Z|] \geq q(C) - 30\epsilon \opt$. 


Let us denote by $Z_r$ the matching returned by $\findmatching{r}{\mc{C}}$. Note that $Z_r$ is a random variable which is a function of both the randomization in realization $\mc{C}$ of $C$, and the internal randomizations used in algorithm $\findmatching{r}{\mc{C}}$.  (Observe that $Z = Z_t$.) Similarly, we define $P_r$, $H_r$, $I_r$, and $P'_r$ as the random variables referring to the values of $P$, $H$, $I$, and $P'$ in algorithm $\findmatching{r}{\mc{C}}$.


Property~1 of Lemma~\ref{lem:independentmatching} is a corollary  of  Lemma~\ref{lem:increaseexp} which states that for any $r$, if $\E[|Z_r|] \leq q(C)-30\epsilon\opt$, then $\E[|Z_r|] -\E[|Z_{r-1}|] \geq \epsilon^5\opt$.  Observe that it is sufficient for us as it implies that for any $r$ we have
$$
\E\big[|Z_t|\big] \geq \min\{q(C) - 30\epsilon \opt,  r\epsilon^5\opt\}.
$$ This gives us the desired result that $\E\big[|Z_t|\big]  \geq q(C) - 30\epsilon \opt$ for $t=1/\epsilon^5$, since $q(C) \leq \opt$. Below we state Lemma~\ref{lem:increaseexp} and prove it.
\begin{lemma}\label{lem:increaseexp}
	For any $r$, if $\E[|Z_r|] \leq q(C)-30\epsilon\opt$, then $\E[|Z_r|] -\E[|Z_{r-1}|] \geq \epsilon^5\opt$.
\end{lemma}
\begin{proof}
This lemma is a direct result of Lemma~\ref{cl:increaseinZisI} and Lemma~\ref{lem:sizeI}. The first one states that for any $r$, we have $\E[|Z_r|] \geq \E[|Z_{r-1}|] + \frac{\E[|I_r|]}{\alpha+1}$ and the second one is that if $\E[|Z_{r-1}|] \leq q(C)-30\epsilon\opt$, then $\E[|I_r|] \geq 2\epsilon^2 \opt$. Combining these two lemmas gives us $\E[|Z_r|] -\E[|Z_{r-1}|] \geq \epsilon^5\opt$ and completes the proof as $\alpha=1/\epsilon$.
\end{proof}

\begin{lemma}\label{cl:increaseinZisI}
	For any $r$, it holds that $\E[|Z_r|] = \E[|Z_{r-1}|] + \frac{\E[|I_r|]}{\alpha+1}$.
\end{lemma}
\begin{proof} We start by proving that 
\begin{equation} \label{eq:md88} \sum_{v\in V} d_{P_r}(v) + 2|I_r| = \sum_{v\in V} d_{P'_r}(v).\end{equation} Note that, $P'_r$ is defined to be the result of iteratively applying all the augmenting hyperwalks of $I_r$ on $P_r$. Let $P^{(i)}_r$ be the result of iteratively applying the first $i$ augmenting hyperwalks of $I_r$ on $P_r$ and let $W_i$ be the hyperwalk that is to be applied in iteration $i$. We use proof by induction and show that for any $i$ we have $$\sum_{v\in V} d_{P_r}(v) + 2i = \sum_{v\in V} d_{P^{(i)}_r}(v).$$
Note that since hyperwalks in $I_r$ are vertex disjoint, for any two hyperwalks $W_1, W_2 \in I_r$ it holds that $W_2$ is an augmenting hyperwalk of $P_r\Delta W_1$ as well. This means that $W_i$ is indeed an augmenting hyperwalk of $P^{(i)}_r$. Moreover, recall that by definition of augmenting hyperwalks, after applying any augmenting hyperwalk on a profile $P$ there are only two vertices whose $d_{P}(v)$ increases by one and for the rest of the vertices it is unchanged. This gives us $$\sum_{v\in V} d_{P^{(i)}_r}(v) + 2 = \sum_{v\in V} d_{P^{(i+1)}_r}(v),$$ with completes the proof of  $$\sum_{v\in V} d_{P_r}(v) + 2|I_r| = \sum_{v\in V} d_{P'_r}(v)$$ since $P'_r = P^{|I_r|}_r$. 
Recall the definition $d_P(v) := \big |\{ i \mid v \in V(M_i) \}\big |$ for any profile $P$. Based on this definition, we can rewrite Equation~\ref{eq:md88} as 

\begin{equation} \label{eq:md99} \sum_{i=0}^{\alpha} |M_i| + |I_r| = \sum_{i=0}^{\alpha} |M'_i|.\end{equation} 

Observe that matchings $M_0, \dots, M_\alpha$ are coming from the same distribution and we have $\E\big[|M_i|\big] = \E\big[|Z_{r-1}|\big]$ for any $0\leq i\leq \alpha$. The reason is that they are the results of running the same matching algorithm on random realizations of $C$. Moreover, by Observation~\ref{obs:samedist}, matchings $M'_0, \dots, M'_\alpha$ are similarly coming from the same distribution which means for any $0\leq i\leq \alpha$ we have $Z_{r} = \E\big[|M'_0|\big] = \E\big[|M_i|\big]$. Combining this with Equation~\ref{eq:md99} we get
$$ \E\big[(\alpha+1)|Z_{r-1}| +|I|\big] = \E\Big[\sum_{i=0}^{\alpha} |M_i| + |I|\Big] = \E\Big[\sum_{i=0}^{\alpha} |M'_i|\Big] = \E\big[(\alpha+1)|Z_r|\big].$$
Dividing through by $\alpha + 1$ and rearranging the terms gives $ \E\big[|Z_{r-1}|\big] +\frac{\E[|I|]}{\alpha+1} =  \E\big[|Z_r|\big]$.
\end{proof}
Before proceeding to Lemma~\ref{lem:sizeI} and its proof we need the following definition.
\begin{definition}[Edge disjoint hyperwalks]
	We say two hyperwalks $W = ((e_1, s_1), \dots, (e_k, s_k) )$ and $W' = ((e'_1, s'_1), \dots, (e'_{k'}, s'_{k'}) )$ are edge disjoint if there does not exist indices $i< k$ and $j< k'$, where $e_i = e'_j$ and $s_i = s'_j$. 
\end{definition}



\begin{lemma} \label{lem:sizeI}
	If $\E[|Z_{r-1}|] \leq q(C)-30\epsilon\opt$, then $\E[|I_r|] \geq 2\epsilon^2 \opt$.
%	For any $r\in [t]$ if $\E\big[|\findmatching{r-1}{\mc{C}}|\big] \leq q(C) - 30 \epsilon^2 \opt$ then expected size of set $I$ in algorithm $\findmatching{r}{\mc{C}}$ is at least $\epsilon^2\opt/4 .$
\end{lemma}

\begin{proof}
	To give the desired lower-bound for $\E[|I_r|]$ we first claim that if $\E[|Z_{r-1}|] \leq q(C)-30\epsilon\opt$ there exists a set $O$ of edge-disjoint augmenting-hyperwalks of $P_r$ with unsaturated end-points where $\E[|O|] \geq8(\alpha+1)\epsilon\opt$. We later state this claim more formally in Lemma~\ref{lemma-size} and provide a  proof for it. We are interested in set $O$ for its two following properties. First, any hyperwalk in $O$ represents a node in graph $H_r$. Second, since the hyperwalks in $O$ are edge disjoint, any hyperwalk with length smaller than $2/\epsilon$ from $P_r$ can share vertices with at most $(\alpha+1)(2/\epsilon)$ hyperwalks in this set. We note that $(\alpha+1)$ is the maximum number of edge disjoint hyperwalks that can pass through a single vertex. Combining these two properties gives that the expected size of any maximal independent set of $H_r$ is at least $\E\big[|O|\big]/(2(\alpha+1)/\epsilon) = 4\epsilon^2\opt$ since there is an edge between two vertices in $H_r$ iff their corresponding hyperwalks share at least a vertex. As stated in Line~\ref{line:setI} of \findmatching{r}{\mc{C}}, set $I_r$ is an independent set of $H_r$ with size at least $(1-\epsilon)$ fraction of a maximal independent set of $H_r$. Therefore, we have $$\E\big[|I_r|\big] \geq 4(1-\epsilon)\epsilon^2\opt.$$ Assuming that $\epsilon\leq 1/2$ we complete the proof of this claim and obtain $\E\big[|I_r|\big] \geq 2\epsilon^2\opt$.
	\end{proof}
	
In the rest of this section we focus on proving the following lemma which is previously used to complete the proof of Lemma~\ref{lem:sizeI}. Since the proof is detailed and consists of independent arguments, it includes two claims that are needed to complete the proof.
 
\begin{lemma} \label{lemma-size}
For any $r\in [t]$, if $\E\big[|Z_{r-1}|\big] \leq q(C) - 30 \epsilon \opt$, then there exists a set $O$ of edge-disjoint augmenting hyperwalks of profile $P_r =  ((\mc{C}_0, M_0), \ldots, (\mc{C}_\alpha, M_\alpha))$ with unsaturated endpoints where $\E[|O|] \geq8(\alpha+1)\epsilon\opt.$ 
\end{lemma}



We will first construct set $O$ and then give a  lower-bound for its expected size. Draw $\alpha+1$ realizations $\mc{N}_0, \dots, \mc{N}_\alpha$ of the non-crucial graph $N$. For any $0\leq i \leq \alpha$, let $M^g_i := M(\mc{N}_i \cup \mc{C}_i)$ where $M$ returns a unique maximum matching that was also used in Algorithm~\ref{alg:sampling}. Call an edge of graph $\mc{C}_i$ \emph{green} iff it is in matching $M^g_i$ but not in matching $M_i$. Alternatively, we call an edge \emph{red} iff it is in $M_i$ but not in $M^g_i$. 
To construct set $O$ we give an algorithm to iteratively find hyperwalks that alternate between green and red edges. Since we need our hyperwalks to be edge-disjoint, after using an edge of a subgraph we mark it as used and ignore it for the rest of the algorithm. 

At each iteration of the algorithm, we construct a hyperwalk $W$ as follows until there is no such a hyperwalk left. Pick an unsaturated vertex $v$ and a subgraph $\mc{C}_i$ such that $v$ has an unused green edge in $\mc{C}_i$ but not a red one. Denote this green edge by $e=(v, v')$ and choose $(e, i)$ to be the first element of our hyperwalk. If vertex $v'$ has a red edge $e'$ in subgraph $\mc{C}_i$ we add $(e', i)$ to our hyperwalk, otherwise we look for a  subgraph $\mc{C}_j$ in which $v'$ has an unused red edge $e'$ but not a green one and choose $(e', j)$ as the second element of the hyperwalk. We continue this process by alternating the colors until it is not possible to continue. Let $u$ be the vertex in which our hyperwalk ends. If $u$ is saturated we add $W$ to a set $T_1$. Otherwise, if the last edge of $W$ is green we add it to $O$ and if it is red we add $W$ to $T_2$. In the following claim we show that the hyperwalks in $O$ have the desired property and we later prove that $|O|$ is large enough.

\begin{claim}
Set $O$ contains edge-disjoint augmenting-hyperwalks that begin and end in unsaturated vertices. 
\end{claim}

\begin{proof}
Any hyperwalk in $O$ begins with an unsaturated vertex and ends in one. Also, hyperwalks in $O$ are edge disjoint since after adding an element $(e, i)$ to a hyperwalk we mark $e$ as used in subgraph $\mc{C}_i$ and do not add it to other hyperwalks. Therefore, we only need to show that any $W = ((e_1, s_1), \dots, (e_k, s_k))\in O$ is an augmenting-hyperwalk. Let $P_r \Delta W$ be the result of applying $W$ on $P_r = ((\mc{C}_0, M_0), \ldots, (\mc{C}_\alpha, M_\alpha))$. By definition~\ref{def:aug}, there are three conditions that $P_r \Delta W$ should satisfy if $W$ is an augmenting-hyperwalk. The first condition is that any $M'_i$ is a matching in $\mc{C}_i$ where
$$
	M'_i = M_i \cup \{ e_j \mid j \text{ is odd, and } s_j = i\} \setminus \{ e_j \mid j \text{ is even, and } s_j = i\}, \qquad \text{for all $i \in \{0, \ldots, \alpha\}$}.
$$
Note that $W$ is alternating between green and red edges with green ones being in the odd positions. Further, for any element $(e, i)$ in an odd position $j$ and any red edge $e'$ adjacent to it in $\mc{C}_i$, hyperwalk $W$ contains $(e', i)$ in either position $j-1$ or position $j+1$; thus the first condition is satisfied.

As for the second condition, since $W$ is alternating between green and red edges applying it would satisfy $d_{P_r}(v) = d_{P_r \Delta W}(v)$ for any vertex $v$ that is not an end-point. Moreover, $P_r \Delta W$ simply satisfies the third condition that is $d_{P_r}(v) + 1 = d_{P_r \Delta W}(v)$ iff $v$ is the first or the last vertex of the hyper-walk since $W$ begins and ends with green edges.
\end{proof}


To complete the proof of Lemma~\ref{lemma-size}, we need to show that $\E[|O|] \geq \alpha\epsilon\opt$. For any vertex $v$ let $g_{v, i}$ be the number of subgraphs $\mc{C}_0, \dots \mc{C}_\alpha$ in which $v$ has an unused green edge after the $i$-th iteration of the algorithm and similarly define $r_{v, i}$ to be the number of subgraphs in which $v$ has an unused red edge after the $i$-th iteration. Each iteration here  means constructing a hyperwalk and marking its edges as used. Also, let us respectively denote the set of saturated and unsaturated vertices by $S$ and $U$. 
Consider the hyperwalk $W_i$ constructed in the $i$-th iteration. Observe that if $W_i\in O$, we have $$\sum_{v\in U} (g_{v, i-1} - r_{v, i-1}) - \sum_{v\in U} (g_{v, i} - r_{v, i}) =2 $$ since any hyperwalk in $O$ starts from an unsaturated vertex with a green edge and ends the same way. However, if $W_i\in T_2$, we have $$\sum_{v\in U} (g_{v, i-1} - r_{v, i-1}) - \sum_{v\in U} (g_{v, i} - r_{v, i}) = 1,$$ and if $W_i\in T_1$ we have $$\sum_{v\in U} (g_{v, i-1} - r_{v, i-1}) - \sum_{v\in U} (g_{v, i} - r_{v, i}) = 0.$$
We claim that when our algorithm stops $\sum_{v\in U} (g_{v} - r_{v}) \leq 0$ holds. Otherwise, we could still find a subgraph $\mc{C}_i$ and a vertex $v$ where $v$ has a green edge in $\mc{C}_i$ but not a red one and start a new hyperwalk. As a result we have the following lower-bound for $|O|$. For brevity, in the rest of the proof we use $g_{v}$ and $r_{v}$ instead of $g_{v,0}$ and $r_{v,0}$.

$$|O| \geq  \frac{1}{2} \Big(\sum_{v\in U} (g_{v} - r_{v}) - |T_2|\Big)$$
Thus,
\begin{equation} \label{eq:m22} \E\big[|O|\big] \geq \frac{1}{2}\E\Big[\sum_{v\in U} (g_{v} - r_{v}) - |T_2|\Big] = \frac{1}{2}\E\Big[\sum_{v\in U} (g_{v} - r_{v})\Big] - \frac{1}{2}\E\big[|T_2|\big].\end{equation}
We first focus on bounding $\E\big[\sum_{v\in U} (g_{v} - r_{v})\big]$ and prove that it is upper-bounded by $40\alpha\epsilon\opt$.

$$\sum_{v\in U} \E[g_{v} - r_{v}\big] =
 \sum_{v\in V} \E[g_{v} - r_{v}\big]  - \sum_{v\in S} \E[g_{v} - r_{v}\big] $$
 Note that $c_v$, by definition, is the probability with which vertex $v$ is matched in any $M^g_i$. Moreover, $\gamma_{v, r}$ is the probability with which vertex $v$ is matched in any $M_i$ which means $\E[g_v - r_v]= (\alpha+1)(c_v-\gamma_{v, r})$ and $$\E\big[\sum_{v\in V} (g_v-r_{v})\big] = 2(\alpha+1) (q(C) - \E\big[|Z_r|\big]).$$ 
 Also, since $ \E\big[|Z_r|\big] \leq q(C) - 30 \epsilon \opt$ we obtain $$\E\big[\sum _{v\in V} g_{v}\big] - \E \big[\sum_{v\in V}r_{v}\big] \geq 60(\alpha+1)\epsilon\opt.$$ Moreover, by definition of saturated vertices, we know that $c_v-\gamma_{v, r} \leq 2\epsilon^2$ holds for any saturated vertex $v$ which results in 
 
 \begin{equation} \label{eq:m-exp}\sum_{v\in S} \E[g_{v} - r_{v}\big] \leq 2n(\alpha+1)\epsilon^2 \leq 20(\alpha+1)\epsilon \opt.\end{equation} Note that $2n(\alpha+1)\epsilon^2  \leq 20(\alpha+1)\epsilon \opt$ comes from Assumption~\ref{ass:optlarge} that $\opt\geq 0.1\epsilon n$. Combining these equation, we get
 
\begin{equation}\label{eq:m33} \sum_{v\in U} \E[g_{v} - r_{v}\big]  \geq 40(\alpha+1) \epsilon \opt.   \end{equation}
In the next step, we provide an upper-bound for $\E\big[|T_2|\big]$ and to do so we first prove the following claim.


\begin{claim}
For any vertex $v \in S$ the number of hyperwalks in $T_2$ that end in $v$ is upper-bounded by $|g_v-r_v|$. 
\end{claim}
\begin{proof}




Consider the hyperwalk $W$ that is the first one to be constructed amongst the hyperwalks that end in vertex $v$ and let $(e, i)$ be its last element. W.l.o.g., assume that the color of edge $e$ in graph $\mc{C}_i$ is red.
The fact that $W$ stops in vertex $v$ means that at the time of construction of this hyperwalk, there is no subgraph $\mc{C}_j$ that has an unused green edge of $v$ but not a red one. Therefore, from this point of the algorithm, any subgraph $\mc{C}_k$ that contains an unused green edge $e_g$ of vertex $v$ also has an unused red edge $e_r$ of this vertex. We note that based on our algorithm if a hyperwalk with last element $(e, i)$ stops at vertex $v$  then subgraph $\mc{C}_i$ either does not contain a green edge of $v$ or a red edge of this vertex. Moreover, due to the fact that $W$ is the first hyperwalk to stop in vertex $v$ we know that previously constructed hyperwalks contain the same number of green and red edges of vertex $v$. This means that there are at most $|g_v-r_v|$ many possibilities for the last element of a hyperwalk that stops at $v$ and since our hyperwalks are edge disjoint then for any vertex $v \in S$ the number of hyperwalks in $T_2$ that end in $v$ is upper-bounded by $|g_v-r_v|$
	\end{proof}
 Based on the aforementioned claim, the number of hyperwalks ending in saturated vertices is at most $\sum_{v\in S} \E[g_v - r_v]$, which means
$$\E\big[|T_2|\big] \leq \sum_{v\in S} \E\big[|g_v - r_v|\big].$$
 We have 
  $$\sum_{v\in S} \E\big[|g_v - r_v|\big] = \sum_{v\in S} \E\big[|g_v - \E[g_v] - r_v + \E[r_v]+ \E[g_v] - \E[r_v]\big] \leq \sum_{v\in S} (\sigma_{r_v} +\sigma_{g_v} + \E[g_v] - \E[r_v]). $$
For the standard deviation of $g_v$ we have $$\sigma_{g_v}  \sqrt{\var(g_v)} \leq \sqrt{(\alpha+1) c_v (1-c_v)} \leq \sqrt{\alpha+1}.$$ It is easy to see that similarly we have $\sigma_{r_v} \leq \sqrt{\alpha+1}$ for any $v$. Since in  \findmatching{r}{\mc{C}}  we set $\alpha=1/\epsilon^3-1$ and since $n\leq 10\opt/\epsilon$ we have $$\sum_{v\in S} (\sigma_{r_v} +\sigma_{g_v}) \leq 2n\sqrt{\alpha+1} \leq 20\opt\sqrt{(\alpha+1)}/\epsilon \leq 20(\alpha+1) \epsilon^{0.5} \opt.$$ 
Moreover, by Equation~\ref{eq:m-exp}, we have $$\sum_{v\in S}(\E[g_v] - \E[r_v]) \leq 20(\alpha+1)\epsilon\opt.$$
As a result we obtain \begin{equation} \label{eq:m44}\sum_{v\in S} \E\big[|T_2|\big] \leq 20(\alpha+1)\epsilon\opt (1 + \epsilon^{-0.5}).\end{equation}
Combining equations \ref{eq:m22}, \ref{eq:m33} and \ref{eq:m44} gives us the following result for the expected size of set $O$.

\begin{equation} \E\big[|O|\big] \geq \frac{1}{2}\E\Big[\sum_{v\in U} (g_{v} - r_{v})\Big] - \frac{1}{2}\E\big[|T_2|\big] \geq (\alpha+1)\epsilon\opt(10-\epsilon^{0.5}). \end{equation} 
 Since  $\epsilon^{0.5} < 1$  we get  $$\E[|O|]\geq 9(\alpha+1)\epsilon\opt\geq 8(\alpha+1)\epsilon\opt,$$
which completes the proof of Lemma~\ref{lemma-size}.



